Weyl's law for singular Riemannian manifolds

We study the asymptotic growth of the eigenvalues of the Laplace-Beltrami operator on singular Riemannian manifolds, where all geometrical invariants appearing in classical spectral asymptotics are unbounded, and the total volume can be infinite. Under suitable assumptions on the curvature blow-up, we show how the singularity influences the Weyl's asymptotics. Our main motivation comes from the construction of singular Riemannian metrics with prescribed non-classical Weyl's law. Namely, for any non-decreasing slowly varying function $\upsilon$ we construct a singular Riemannian structure whose spectrum is discrete and satisfies \[ N(\lambda) \sim \frac{\omega_n}{(2\pi)^n} \lambda^{n/2} \upsilon(\lambda). \] Examples of slowly varying functions are $\log\lambda$, its iterations $\log_k \lambda = \log_{k-1}\log\lambda$, any rational function with positive coefficients of $\log_k \lambda$, and functions with non-lo\-ga\-rithmic growth such as $\exp\left((\log \lambda)^{\alpha_1} \dots (\log_k \lambda)^{\alpha_k} \right)$ for $\alpha_i \in (0,1)$. A key tool in our arguments is a new quantitative estimate for the remainder of the heat trace and the Weyl's function on Riemannian manifolds, which is of independent interest.

==> aR.tex <==
\subsection{Regular almost Riemannian structures}

\begin{definition}
  A singular Riemannian structure on an $n$-dimensional manifold $N$ is \emph{regular} of order $m$ if there exists $\phi$ such that
  \begin{equation}
    \det a_{ij}(x,z) = x^m\phi(x,z), \qquad \phi(x,z)\neq 0.
  \end{equation}
\end{definition}

\begin{prop}
  Any convex and regular ARS on a compact manifold $N$ satisfy assumption $\Sigma$.
\end{prop}

\begin{proof}
	Let $C=a^{-1}\partial_xa$ and recall that $\Hess(\distmb)=-(C+C^*)/2$.
	By the well-known formula $\partial_x\det a = \det a \operatorname{tr}C$, we immediately get that $\operatorname{tr}\Hess(\distmb)=-\operatorname{tr}(C) = -\phi(x,z)/x$ and $\operatorname{tr}\partial_x\Hess(\distmb)=\psi(x,z)/x^2$for some smooth $\phi,\psi\neq0$. Thanks to the convexity,  this implies that $\Hess(\distmb)\ge -b/\delta$ for some $b>0$. Finally, exploiting the Riccati equation connecting Hessian and curvature, this implies th
\end{proof}


\subsection{Regular almost Riemannian structures}

\begin{definition}
  A singular Riemannian structure on an $n$-dimensional manifold $N$ is \emph{regular} of order $m$ if there exists $\phi$ such that
  \begin{equation}
    \det a_{ij}(x,z) = x^m\phi(x,z), \qquad \phi(x,z)\neq 0.
  \end{equation}
\end{definition}


We have the following.

\begin{prop}
  For any convex and regular ARS on a compact manifold $N$ there exists a splitting $TZ=\mathcal D_1\oplus\ldots\oplus\mathcal D_N$, where $\mathcal D_1,\ldots,\mathcal D_N$ are smooth vector distributions, and exponents $0\le m_1<\ldots<m_N$ such that
  \begin{equation}
    g = dx^2 + \sum_{i=0}^{N}x^{-2i}h_i(x).
  \end{equation}
  Here, $h_i(x)$ are one-parameter families of Riemannian metrics on $\mathcal D_i$, smooth up to $x=0$, and $\sum_{i=0}^Nm_i=m$.
\end{prop}


\begin{proof}
  By compactness of $N$, it is enough to prove the statement locally. Namely, recalling that $g=dx^2+(a^*a)^{-1}dz^2$, we will show that there exists local coordinates at $p\in Z$ such that
  \begin{equation}\label{eq:claim-ars}
    a^*a(x,z) = A(x,z)\sum_{i=0}^{N} x^{-2m_i}\pi_i.
  \end{equation}
  Here, $\pi_i:\R^{n-1}\to \R^{n-1}$ are projections such that $\sum_{i=0}^m\pi_i=\idty$, $\sum_{i=0}^N m_i = m$, and the matrix $A\in C^{\infty}$ is symmetric positive-definite, invertible at $0$, and block-diagonal w.r.t.\ the projections $\pi_i$, i.e., $\pi_k A \pi_\ell=0$ if $k\neq\ell$.


  By convexity, we have that $\partial_x(a^* a)\ge 0$ in the sense of symmetric forms.
  Thanks to  the regularity assumption, the preparation theorem for matrix valued functions \cite[Theorem~5.3]{Dencker1993} yields, for some $N\le 2m$,
  \begin{equation}\label{eq:preparation}
    a^*a(x,z) = A(x,z) \left( d(x) + \sum_{j=0}^{N-1}x^jB_j(z) \right).
  \end{equation}
  Here, $A$ is a smooth matrix valued functions such that $\det A(0,0)\neq0$, $d(x) = \sum_{i=0}^{N} x^i\pi_i$, $\sum_{i=0}^N\pi_i=\idty$, and $B_j\pi_k=0$ if $j\geq k$. Up to a change of coordinates, we can always assume $A(0,0)=\idty$.
  
  Letting $D_0=\sum_{i=0}^{N} i \pi_i$, we have $d^{-1}\partial_xd=x^{-1}D_0$, so that
  \begin{equation}
    \partial_x(a^*a)=\frac 1x\left( AdD_0 + A\sum_{j=1}^{N-1}jx^jB_j+ x\partial A \left(d+\sum_{j=0}^{N-1}x^jB_j  \right) \right).
  \end{equation}
  Writing $A=\idty+x\tilde A$ for some regular $\tilde A$, the positive semi-definiteness of $\partial_x(a^*a)$ implies that, for $x$ sufficiently small, it holds\todo{Is it sufficient to explain it like this?}
  \begin{equation}
    v^*\left(dD_0 + \sum_{j=1}^{N-1}jx^jB_j\right)v\ge 0, \qquad \forall v\in\R^n.
  \end{equation}
  In particular, we obtain $\pi_\ell B_j\pi_k=-\pi_k B_j\pi_\ell$ for all $\ell\neq k$. Since $B_j\pi_k=0$ if $j\geq k$, this yields $B_j\equiv 0$ for all $j$'s.
  
  We are now left to prove that $A$ is symmetric, positive-definite, and block-diagonal. Since $B_j\equiv0$ \eqref{eq:preparation} we have
  \begin{equation}
    a^*a = A d, \qquad 
    \partial_x(a^*a)=\frac {1}xA^{-1}\left( D_0 +  xA^{-1}\partial M   \right)d.
  \end{equation}
  In particular, $A$ is symmetric and $A\ge 0$ for sufficiently small $x$. Thus, the convexity implies that $D_0 +  xA^{-1}\partial A\ge 0$ for $x>0$. The same computations as above yield that $A$ has to be blockwise anti-symmetric, which implies $\pi_k A \pi_\ell=0$ if $k\neq \ell$.  
  Finally, the smoothness of the matrix $a$ at $0$ implies that the exponents in $d$ are necessarily even, thus completing the proof of \eqref{eq:claim-ars}.
%  
%  Finally, the smoothness of the matrix $a$ at $0$ implies that, renaming $\pi_i=\pi_{2i}$ and letting $\pi_i=0$ if $i>N/2$ we have $d=\sum_{i=0}^{m}x^{2i}\pi_i$. Inverting the resulting block-diagonal expression for $a^*a$ yields the statement.
\end{proof}

{\blue Non regular ARS. Hypotheses to be stated exactly.

Write (slightly different from the previous definition where $C$ is the transpose and $\partial_0=()_x$)
$$
C:=a^{-1} a_x=\gamma+\beta,\ \gamma = \frac{1}{2}(C+C^*),\ \beta = \frac{1}{2}(C-C^*).
$$
Set now 
\begin{equation}\label{eqY-0}
a=NR,
\end{equation}
where 
$$
R_x=-R\beta, 
$$
is a rotation matrix. One deduces at once that
$$
N_x=N\gamma_R, \ \gamma_R:=R\gamma R^*\hbox{ and }
N^2=aa^*,
$$
implying that $N$ itself is symmetric. Note that $N$ is not necessarily definite positive (so \eqref{eqY-0} is not a polar decomposition but, if $N=R_ND_NR_N^*$ with $R_N$ orthogonal and $D_N$ diagonal, then $a=R_N(\vert D_N\vert)^{1/2}$ is the polar decomposition).
Since $R=N^{-1}a$, its entries are rational fractions in $1/x$ hence can be written as $\frac{\alpha(x)}{x^m}$ with $\alpha(0)\neq 0$.

TO BE JUSTIFIED. has to avoid $\exp(-1/x^2)$...

Since the coefficients of $R$ are bounded we deduce that each exponent $m$ in $\frac{\alpha(x)}{x^m}$ must be non zero.
Hence both $R$ and $R^{-1}$ have smooth entries. Then 
$\beta$ has smooth entries and $C$ as well. We are done


}

==> preliminaries.tex <==
\section{Preliminaries}

In this section we collect some basic definitions and notations used in the rest of the paper. {\red In particular, the notions presented in Section~\ref{s:bdry} will be used for the heat kernel and trace estimates of Section~\ref{s:heat}, while those presented in Section~\ref{s:non-complete} will be used in Sections~\ref{s:weyl} and \ref{s:ARS}.}

\subsection{Riemannian manifolds with boundary}\label{s:bdry}

Let $(M,g)$ be a smooth $n$-dimensional Riemannian manifold, with smooth boundary $\partial M$. We let $\distb:M\to [0,+\infty)$ be the Riemannian distance from $\partial M$, that is,
\begin{equation}
  \distb(x) = \inf_{z\in\partial M} d(x,z).
\end{equation}
A {\blue length-parametrized} geodesic $\gamma:[0,t]\to M$, $\gamma(0)\in \partial M$ is optimal\todo{L: I would replace ``optimal'' with ``shortest'' or ``minimal'' everywhere.} w.r.t.\ the boundary if for all $0\leq s<t$ it holds $\distb(\gamma(s))=s$. {\red and $\gamma(0)$ is the only point of ${\partial M}$ realising $\distb(\gamma(s))$.} In particular, it necessarily holds that $\dot\gamma(0)\perp T_{\red{z}\blue{\gamma(0)}}\partial M$, {\blue and $\gamma(0)$ is the unique closest point on $\partial M$ to $\gamma(s)$}.

\begin{definition}
  The \emph{injectivity radius at $x\in M$}, denoted by $\inj_M(x)$ is the supremum of times $t>0$ such that every optimal geodesic emanating from $x$ is either optimal up to time $t$ or crosses the boundary at some time $t'<t$. The \emph{injectivity radius of $M$} is then equal to
  \begin{equation}
    \inj_M = \inf_{x\in M} \inj_M(x).
  \end{equation}
  The \emph{injectivity radius from $\partial M$ at $z\in \partial M$}, denoted by $\inj_{\partial M}(z)$, is defined similarly, by replacing optimal geodesics with optimal geodesics w.r.t.\ the boundary.
  We then let the \emph{injectivity radius of $\partial M$} to be
  \begin{equation}
    \inj_{\partial M} = \inf_{z\in \partial M} \inj_{\partial M}(z).
  \end{equation}
\end{definition}
{\red Observe that, with the above definition, $\inj_M>0$ for any compact manifold. Moreover, if $M$ is a bounded smooth open subset of $\R^d$, then $\inj_M=+\infty$.
In general, it could happen that $\inj_{\partial M} = 0$ (e.g., for the Euclidean square in $\R^n$). }

{\blue It is well known that $\distb$ is smooth on $\{ \distb < \inj_{\partial M}\}$, and that the level sets $Z_\varepsilon = \{\distb = \varepsilon\}$ are smooth embedded hypersurfaces for $\varepsilon \in [0,\inj_{\partial M})$.}

For a smooth function $f:M\to \R$, we {\blue let} {\red denote by $\Hess(f)$ the Riemannian Hessian of $f$, that is, }
\begin{equation}
  \Hess(f)(X,Y)=g(\nabla_X \nabla f, Y),\qquad X,Y\in \Gamma(M),
\end{equation}
where $\nabla$ denotes the covariant derivative. {\red In the following, t} The notation $\Hess(f)\ge c$ (resp.\ $\le c$) for some constant $c\in\R$ is to be understood in the sense of quadratic forms and w.r.t.\ the metric $g$.

{\red Let {$0<\varepsilon<\inj_{\partial M}$.} Notice that $\distb$ is smooth on $\{\distb<\inj_{\partial M}\}$, and thus $Z_\varepsilon=\{\distb = \varepsilon\}$ is a smooth embedded hypersurface. The second fundamental form and the mean curvature of $Z_\varepsilon$ are equal to $\Hess(\distb)|_{TZ_{\varepsilon}}$ and its trace, respectively.}


\begin{definition}
  The boundary $\partial M$ is convex (resp.\ strictly convex) if its second fundamental form $\Hess(\distb)|_{\partial M}$  is non-positive (resp.\ negative). Moreover, it is mean convex if $\tr \Hess(\distb)|_{\partial M} \le 0$.
\end{definition}

\todo[inline]{L: In the next section is not clear what $\Omega$ is. Sometimes $M$ appeared. Are we introducing all our objects already in the non-complete case, or are we still in the setting of Section 2.1?  I replaced some $M$ with $\Omega$ for consistency, having in mind that $\Omega$ can be a complete manifold with boundary $\Omega = \mathcal{M}_\varepsilon$, a compact manifold $\Omega = \bar{M}$, a non-complete manifold $\Omega = \mathcal{M}$, an open set of a non-complete manifold as in Proposition \ref{p:resolvent}). There are also some repetitions with Section 2.2 below. I will go back to this section after you checked it.}


\paragraph{Laplace-Beltrami operator.} We use $L^2(\Omega)$ to denote the space of square integrable functions on $\Omega$ w.r.t.\ the Riemannian measure $d\mu_g$.
For any $u\in L^2(\Omega)$, we let $\nabla u$ be the distributional Riemannian gradient of $u$, and define its $H^1$ norm as
\begin{equation}
  \|u\|_{H^1(\Omega)}^2 = \int_{{\red M} {\blue \Omega}} |u|^2\,d\mu_g + \int_{{\red M} {\blue \Omega}}|\nabla u|^2\,d\mu_g.
\end{equation}
Then, $H^1_0(\Omega)$ and $H^1(\Omega)$ are, respectively, the closure of $C^\infty_c(\Omega)$ and of $\{u\in C^\infty(\Omega)\mid \|u\|_{H^1(\Omega)}<+\infty\}$ w.r.t.\ this norm. 
{\red We remark that $H^1(\Omega)\subset W^1(\Omega)$, where the latter is the space of $L^2(\Omega)$ functions with distributional gradient in $L^2(\Omega)$.} \todo{L: It seems to me that $W^1$ is used only in the reference to Grigoryan for the compact embedding, maybe put that only there (I put a footnote there)}

The Laplace-Beltrami operator is the differential operator defined {\blue on smooth functions} 	by
\begin{equation}\label{eq:laplace-beltrami}
  \Delta  = \operatorname{div}_{\mu_g} \circ \nabla .
\end{equation}
We will consider two realizations of the Laplace-Beltrami operator as an operator on $L^2(\Omega)$: the Friedrichs (or Dirichlet) and the Neumann Laplace-Beltrami operators, denoted, by $\Delta^-_\Omega$ and $\Delta^+_\Omega$, respectively. These are the operators associated with the non-negative symmetric form
\begin{equation}
  \mathcal E (u,v)  = \int_{{\red M} {\blue \Omega}} g(\nabla u,\nabla v)\,d\mu_g,
\end{equation}
with {\blue form} domains $H^1_0(\Omega)$ and $H^1(\Omega)$, respectively.  {\red When $\Omega= M$, we will often drop the subscript, i.e., $\Delta^\pm=\Delta^\pm_{M}$.}\todo{What is $M$ here?}

\begin{rmk}
{\red Let $\Omega=M$. When $M$ is complete,} {\blue If $\Omega$ is a complete Riemannian manifold without boundary,} both the Friedrichs and Neumann Laplace-Beltrami operators coincide since the Laplace-Beltrami operator with domain $C^\infty_c(M)$ is essentially self-adjoint \cite{Gaffney1954}. On the other hand, if $\Omega {\red \subset M}$ {\red is a smooth domain} {\blue has non-empty smooth boundary}, these corresponds to consider Dirichlet and Neumann boundary conditions, respectively.  
\end{rmk}

\paragraph{Heat kernel.}

The Dirichlet (resp.\ Neumann) heat kernel of {\blue $\Omega$} {\red $M$}, denoted by $p^-_{\blue \Omega}$ (resp.\ $p^+_{\blue \Omega}$) is the minimal fundamental solution of the heat equation associated with the Dirichlet (resp.\ Neumann) Laplace-Beltrami operator, i.e.,  $p^\pm_{\blue \Omega}:\R_+\times \Omega\times \Omega\to \R$ is a smooth function such that 
\begin{equation}
  \partial_{t} p^\pm_{\blue \Omega}(t,x,\cdot)=\Delta_\Omega^\pm p^\pm(t,x,\cdot), \qquad \lim_{t\to 0}p^\pm_{\blue \Omega}(t,x,\cdot) = \delta_x, \qquad \forall x\in {\red M} {\blue \Omega}.
\end{equation}
Here, $\delta_x$ denotes the Dirac delta mass at $x\in {\red M} {\blue \Omega}$. In particular, since ${\red M} {\blue \Omega}$ has smooth boundary, the definition of $\Delta_\Omega^\pm$ implies that $p^-_{\blue \Omega}$ satisfies Dirichlet boundary conditions at $\partial {\red M} {\blue \Omega}$, while $p^+_{\blue \Omega}$ satisfies Neumann ones.

\paragraph{Spectrum.}

If $\Omega$ is {\red a relatively} compact {\red set in $M$},  the spectrum of $-\Delta^\pm_\Omega$ is a discrete subset of the positive real axis, i.e., $\sigma(-\Delta^\pm)\subset [0,+\infty)$, accumulating at infinity.  The Weyl counting function is then defined as
\begin{equation}
  N^{\pm}_\Omega(\lambda)=\#(\sigma(-\Delta_\Omega^\pm)\cap [0,\lambda]).
\end{equation}
When $\Omega= \mathcal{M}$, we will always consider the Friedrichs Laplace-Beltrami operator, and denote its Weyl counting function by $N(\lambda)$.\todo{L: what about the non-complete case?}

\subsection{Non-complete Riemannian manifolds}\label{s:non-complete}

Let $\mathcal M$ be a non-complete Riemannian manifold (without boundary).
We let $\widehat{\mathcal M}$ be the metric completion of $\mathcal M$ w.r.t.\ the Riemannian distance and $\partial \mathcal M=\widehat{\mathcal M}\setminus\mathcal M$ be the \emph{metric boundary}. 
The distance from the metric boundary is denoted by $\distmb$. We recall that $\distmb$ is Lipschitz and satisfies the eikonal equation, i.e., $|\nabla\distmb|\equiv 1$.
For any $0\le a<b\le +\infty$, we let $\mathcal M_a^b=\{a\leq \distmb \leq b\}\cap \mathcal{M}$ and $\mathcal Z_a=\{\distmb=a\}$. 

We also assume that $\mathcal M$ has regular metric boundary (in the sense of Definition~\ref{def:regular}), i.e., there exists $\varepsilon_0 >0$ such that $\distmb$ is smooth on $\mathcal{M}_0^{\varepsilon_0}$.
Under this assumption the level sets $\mathcal{Z}_\varepsilon$ are smooth embedded hypersurfaces for all $\varepsilon \in (0,\varepsilon_0]$, and there exists a uniform tubular neighborhood of the metric boundary $\mathcal{M}_0^{\varepsilon_0} \simeq (0,\varepsilon_0] \times  \mathcal{Z}_{\varepsilon_0}$ where the metric reads
\begin{equation}\label{eq:collar}
g  = dx^2 + h_x(z), \qquad (x,z) \in (0,\varepsilon_0] \times \mathcal{Z}_{\varepsilon_0}.
\end{equation}
Here, $h_x$ is a one-parameter family of smooth metrics on $\mathcal{Z}_{\varepsilon_0}$. Within this identification, $\distmb(x,z) = x$. Furthermore for all $\varepsilon \leq \varepsilon_0$ the truncation $\mathcal{M}_\varepsilon^\infty$ admits an inward tubular neighborhood of its boundary, given by $\mathcal{M}_\varepsilon^{\varepsilon_0}$, on which the metric is the restriction of \eqref{eq:collar} to $(\varepsilon,\varepsilon_0]\times \mathcal{Z}_{\varepsilon_0}$. Hence, the distance from its boundary $\partial \mathcal{M}_\varepsilon^\infty = \mathcal{Z}_\varepsilon \simeq \mathcal{Z}_{\varepsilon_0}$,  satisfies 
\begin{equation}
\distb(x,z) =  \distmb(x,z)-\varepsilon  = x-\varepsilon.
\end{equation}
We reformulate this last statement in an equivalent way, as follows.
\begin{lemma}[Boundary injectivity radius estimate]
Let $\mathcal{M}$ be a non-complete Riemannian manifold with regular metric boundary. Then, up to halving $\varepsilon_0$, it holds\todo{L: I do not like this ``halving'' in the statement. I would put $\varepsilon_0/2$ here.}
\begin{equation}
\inj_{\partial M_\varepsilon^\infty} \geq \varepsilon_0, \qquad \forall \varepsilon \leq \varepsilon_0.
\end{equation}
\end{lemma}

From now on, we assume $\mathcal M$ to have compact metric completion.
{\red On $\mathcal M$ we are only interested in the Friedrichs Laplace-Beltrami operator, as defined in the previous section, that we denote simply by $\Delta$. In particular, we will consider only the Sobolev space $H^1_0(\mathcal M)$.

 For this reason, given $\Omega\subset \mathcal M$, we define the Sobolev space $H^1_0(\Omega)$, as in the case of manifolds with boundary, to be the closure of $C^\infty_c(\Omega)$ w.r.t.\ the $H^1(\Omega)$ norm, and $H^1(\Omega)$, to  be the closure w.r.t.\ the same norm of the set\footnote{By $C^\infty(\Omega)\cap C^\infty_c(\mathcal M)$ we mean functions on $\Omega$ that are restrictions of functions of $C^\infty_c(\mathcal M)$.} $C^\infty(\Omega)\cap C^\infty_c(\mathcal M)$. With this definition, functions of $H^1(\Omega)$ are restrictions of functions of $H^1_0(\mathcal M)$.
Observe that, if $\Omega\subset \mathcal M_\varepsilon^\infty$ for some $\varepsilon>0$ and $\partial \Omega$ is smooth, by \cite[Theorem~2.9]{Aubin}  we recover the definition of $H^1(\Omega)$ given in the case of manifolds with boundary.}\todo{L: repetition of section 2.1?}

We need the following result, that we prove in Appendix~\ref{a:discreteness}.

\begin{prop}[Hardy inequality]\label{p:hardy}
Assume that there exists $\varepsilon_0>0$ such that the boundary of $\mathcal M_\varepsilon^\infty$ is mean convex for any $0<\varepsilon\le \varepsilon_0$. Then, for any $0<\varepsilon\le \varepsilon_0$,
\begin{equation}\label{eq:hardy-boundary}
\int_{{\mathcal M}_0^\varepsilon} |\nabla u|^2 d\mu_g \geq \frac{1}{4} \int_{{\mathcal M}_0^\varepsilon} \frac{|u|^2}{\distmb^2} d\mu_g, \qquad \forall u \in  C^\infty_c({\mathcal M}_0^\varepsilon).
\end{equation}
\end{prop}

Assume from now on that that there exists $\varepsilon_0>0$ such that the boundary of $\mathcal M_\varepsilon^\infty$ is mean convex for any $0<\varepsilon\le \varepsilon_0$. Then, since $\mathcal M$ has compact metric completion, the spectrum of $-\Delta$ is a discrete subset of the positive real axis, i.e., $\sigma(-\Delta^\pm)\subset [0,+\infty)$, accumulating at infinity. (See Proposition~\ref{p:resolvent}.) 
We denote the Weyl counting function associated with $\Delta$ by $N(\lambda)$ and, for $0\le a<b\le\infty$, the Weyl counting function of $\Delta^\pm_{{\mathcal M}_a^b}$ by $N_{[a,b]}^\pm(\lambda)$.\todo{Maybe unify with the ``spectrum'' part of Section 2.1?}

{\red A classical tool to study $N(\lambda)$ is the following, see \cite[p.\ 407]{CH-methods}. }

{\blue We will need the following instance of Dirichlet-Neumann bracketing (see \cite[p.\ 407]{CH-methods}), adapted to our setting.}

\begin{prop}[Dirichlet-Neumann bracketing]\label{p:d-n}
  Let $\mathcal M$ be a non-complete Riemannian manifold with compact metric completion and regular metric boundary. Assume, moreover, that there exists $\varepsilon_0>0$ such that the boundary of $\mathcal M_\varepsilon^\infty$ is mean convex for any $0<\varepsilon\le \varepsilon_0$.
  Then, for any $0=a_0<a_1<\ldots<a_{n+1}=+\infty$, we have
  \begin{equation}
    \sum_{i=0}^n N^-_{[a_i,a_{i+1}]}(\lambda)\le N(\lambda)\le \sum_{i=0}^n N^+_{[a_i,a_{i+1}]}(\lambda) , \qquad \forall \lambda\ge0.
  \end{equation}
\end{prop}

\todo[inline]{L: After having read it, I have some remarks on the structure of this section 2. 1) It is not evident that the only non-standard and perhaps subtle part is when we deal with a non-complete Riemannian manifold possibly with boundary (such as $\mathcal{M}_0^\varepsilon$ or $\mathcal{M}_\varepsilon^\infty$). 2) I believe that everything can be presented at the same time for a general $\Omega$, possibly non-complete and possibly with boundary. For the spectrum statement, the only assumption is that the metric completion of $\Omega$ should be compact and with convex metric boundary. 3) This section contains mostly known definitions or precisations for the non-complete case. Shall we perhaps put the first part of Section 2.1 at the beginning of section 3, and delay the whole non-complete stuff after section 3?}

